Spontaneous Reward Hacking in Iterative Self-Refinement

Language models are capable of iteratively improving their outputs based on natural language feedback, thus enabling in-context optimization of user preference. In place of human users, a second language model can be used as an evaluator, providing feedback along with numerical ratings which the generator attempts to optimize. However, because the evaluator is an imperfect proxy of user preference, this optimization can lead to reward hacking, where the evaluator's ratings improve while the generation quality remains stagnant or even decreases as judged by actual user preference. The concern of reward hacking is heightened in iterative self-refinement where the generator and the evaluator use the same underlying language model, in which case the optimization pressure can drive them to exploit shared vulnerabilities. Using an essay editing task, we show that iterative self-refinement leads to deviation between the language model evaluator and human judgment, demonstrating that reward hacking can occur spontaneously in-context with the use of iterative self-refinement. In addition, we study conditions under which reward hacking occurs and observe two factors that affect reward hacking severity: model size and context sharing between the generator and the evaluator.

==> figtext/author_vs_judge.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.92\textwidth]{figures/author_vs_judge_TEMP.pdf}
    \caption{\redtext{Update caption and figure}. The prompts for author vs. judge. Note that the history allows the judge and the AI author to have access to all the previous iterations of essays and ratings. \jane{need to update this caption}. }
    \label{fig:author_vs_judge}
\end{figure*}


==> sections/shi_old_text.tex <==

% \section{Validating the existence of \aaa{}}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/polish_and_screen.pdf}
%     \caption{One underlying model is used on both ends of the interaction: polishing and screening a resume.}
%     \label{fig:polish_and_screen}
% \end{figure}

% \vspace{-0.2cm}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/exp_overview.pdf}
%     % \caption{We consider two scenarios to be evidence for \aaa: judge rates the AI author higher than the human author when the two are of equal quality according to the oracle; judge rates the AI author and the human author as equal when the human is rated higher by the oracle.}
%     \label{fig:exp_overview}
% \end{figure}
% \vspace{-0.3cm}
% We consider the scenario above to be evidence for \aaa{}: the judge rates the AI author and the human author as equal, while the human is rated higher by the oracle.

% To validate \aaa{}, we design various context for the author--judge interaction which leads to one of the two scenarios.
% The context reported here are biased because they are constructed and selected based on whether \aaa{} is observed successfully.
% But we make it a priority to ensure that the context is plausible in spontaneous interactions between two models, i.e., not too adversarial.


% We explain the \aaa{} in this specific interaction protocol using the analogy of a zipper (Figure~\ref{fig:zipper}).
% At the beginning, although the author and the judge are given the same rubric, they are still not fully aligned in their judgment of what's a good essay due to having different instructions in their prompts.
% But because the two share the same dialogue, their prompts converges, and portion that's unique to each shrinks over time.
% This allows them to converge to a consensus on what's a good essay---a consensus that's not fully aligned with human judgment represented by the oracle.

% The lack of robustness affects both the judge and the author, and our hypothesis is that they tend to exploit the same shortcuts and spurious correlations in the training data---a property that comes to the surface as the shared dialogue history constitutes a larger and larger proportion of their prompts.
% We hypothesize that the process of the judge and the author talking to each other creates an implicit optimization pressure that drives them towards a shared adversarial example, where both the author and the judge make incorrect judgments about the essay's quality.
% Section~\ref{sec:reward_hacking} takes a deeper dive on this hypothesis and validates it empirically.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/zipper.pdf}
%     \caption{The author and the judge are based on the same underlying language model but they start out with two different prompts. As the dialogue between them goes on, their prompts converge, so does their judgment of what's a good essay---like a zipper.}
%     \label{fig:zipper}
% \end{figure}

% \subsection{\aaa{} in individual judgments}

% Although we indeed observe \aaa{} in the shared dialogue setting, the strength of \aaa{} is nonetheless confounded by the zipper effect.
% We now present experiments to expose \aaa{} when the judge only sees one essay at a time, without any dialogue history or context.


% \subsection{Varying the degree of AI involvement in authoring}

% The AI author optionally collaborates with a human author, e.g., by the human author first writing the text which then gets polished by the AI author.
% We refer to the human-AI team collectively as the author, where the AI’s involvement can vary from zero to a hundred percent. 
% The judge is never informed of the level of AI author’s involvement in producing the input, and the key task for the judge is to infer that.
% Both the judge and the AI author will be GPT-series models, meaning they will have significant parameter sharing.
% And because this parameter sharing, our hypothesis is that despite the judge only have black-box access to the author, it actually has white-box access for free.

% Experiment design dimensions:
% We will vary the level of AI author’s involvement along the following dimensions:
% The co-authoring interaction protocol (e.g., AI author writes everything vs. AI post-edit)
% The AI author’s instruction
% This can be roughly thought of as controlling parameter sharing between the judge and the author (although we can’t really count the parameters of the human author). But it gives us a sense of how much theoretical white-box access the judge has over the author.

% \section{\aaa{} is caused---at least partly---by the recognition of the other AI}
% \label{sec:causal}

% AAA can be decomposed into two steps: prove that LM has latent knowledge about whether an input is generated by another LM, and show that such latent knowledge correlates with some notion of preference. Just doing the second step is probably good enough: to show that there is correlation between some notion of preference and the degree to which an LM is involved in the generation of the input. But the point is definitely stronger if we can also establish the first point.

% The fact that detection works reasonably well kind of already shows the first point: that the information of whether an input is produced by LM can be effectively extracted from the LM itself with various methods based on perplexity. So in a sense we can already say that LM has latent knowledge about whether the input is LM-generated. If we can show that such latent knowledge can be surfaced, i.e., getting the LM to output such latent knowledge itself instead of relying on an external algorithm, we have a stronger argument that such latent knowledge can in fact affect LM outputs. This is the point of trying to do zero-shot detection in this project.

% Can the judge recognize the level of AI author’s involvement with only black-box access (i.e., only seeing the author’s output)? We will instruct the judge to do zero-shot detection.

% We will experiment with ways to enhance the white-box access of the judge, by “making the judge more aware of its white-box access”. We will expose the judge’s own logits to the judge, or allow the judge to query a copy of itself to get the logits.
% We will compare all this against external detection tools (which also largely rely on logits of a model with black-box access to the author). We will then try to see if we can few-shot teach the judge to do detection with supervision from these external tools.
% We will measure, given the judge’s inference (under one of the conditions mentioned above), how does that influence the judge’s decision.

% \section{Spontaneous reward hacking through free white-box access}
% \label{sec:reward_hacking}

% When two similar models talk to each other, they get white-box access for free

% Are their gradients aligned?


% \section{\aaa is not at odds with bypass}
% \label{sec:bypass}

% The existence of over-appreciation is somewhat in conflict with the possibility of bypass. The goal of bypass is to make an AI authored text undetectable while maintaining quality. Consider the following experiment: compare the judge’s score on 1) AI authored article vs. 2) the same article but passed through a detection bypass tool. If bypass worked as intended, then the judge should consider them to have the same quality, meaning no over-appreciation. These pairs of [AI text, bypassed version] are basically counterexamples to over-appreciation, where the human text (from the judge’s perspective) is of the same quality as the AI text (assuming judge’s latent knowledge of which is more AI and which is more human). But I would argue that bypass is basically a white-box adversarial attack against over-appreciation, and that if we look at less adversarial conditions where the more human text (from the judge’s perspective) is not constructed specifically to fool the judge, over-appreciation can still happen.

% \section{Planning for a predictable future}
% \label{sec:predictability}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/hacking.pdf}
%     \caption{Reward hacking happen over the course of a dialogue.}
%     \label{fig:hacking}
% \end{figure}


% \section{Inconsistent behaviors of LMs}
% \label{sec:inconsistency}

% Snowball

% \section{\aaa{} and compression}
% \label{sec:compression}

% In the Smallville experiments~\citep{park2023generative}, the reflection process which synthesized all past experience (in text) and dialogue history is shown to improve agent performance. Reflection could have produced a interaction history that’s easier to process for both humans and AIs, but it could also have been acting as a compressor that makes the interaction history easier for just the AIs, which in turn frees up the AI to use its capacity for other behaviors, such as planning.


% We hypothesize that AIs---more specifically language models---have some inherent ``preferences'' for texts generated by similar models.
% Specifically, we consider the interaction between two language models: the \textit{judge}, which is tasked to do scoring (e.g., essay scoring, resume screening), and the \textit{author}, which produces the texts for the judge to score.
% We define preference in the narrow sense and specific to each task.
% In essay scoring, for example, we observe such preference if the judge AI consistently scores essays by an AI author higher than a human author, even when the two write equally well.
% % We call this phenomenon \textbf{Algorithmic Algorithmic Appreciation} (\aaa{}, in short).
% % The name is derived from algorithmic appreciation---the psychological effect of people preferring algorithmic judgment over human judgment.
% % Algorithmic algorithmic appreciation is the phenomenon where an algorithm exhibits that bias.
% We call this phenomenon \aaa.

% \aaa{} can be seen as \textit{spontaneous} reward hacking.
% Typically, reward hacking happens under optimization.
% For example, the author might learn from the judge's feedback as a proxy for human judgment to improve generation quality.
% When optimized for many iterations, the author typically gets higher and higher scores from the judge but it eventually diverges from actual human judgment.
% In a different scenario, a malicious author can use adversarial attack methods to optimize towards a higher score from the judge by exploiting the judge's weaknesses (by peeking at its gradients).
% Our hypothesis is that even without external optimization pressure, reward hacking can occur simply by having the two models talking to each other.
% Section~\ref{sec:reward_hacking} discusses the connection between \aaa{} and reward hacking in more detail.
% % Similar behaviors in AI have been studied in the context of adversarial attacks, steganography (https://arxiv.org/abs/1712.02950, https://arxiv.org/abs/1909.01496), and red-teaming (https://arxiv.org/abs/2202.03286).

% % The second reason why \aaa{} can occur is based on the premise that model-generated text overall is more predictable than human-written ones, even when it’s generated from a different context (e.g., under a different prompt).
% % Higher predictability means AI text leaves a smaller memory footprint for the judge, and we hypothesize that this leads to certain advantages.
% % Model-polished resume is easier to process for AI because it’s already processed by the model once.


